Tracking the Takes and Trajectories of English-Language News Narratives across Trustworthy and Worrisome Websites

Understanding how misleading and outright false information enters news ecosystems remains a difficult challenge that requires tracking how narratives spread across thousands of fringe and mainstream news websites. To do this, we introduce a system that utilizes encoder-based large language models and zero-shot stance detection to scalably identify and track news narratives and their attitudes across over 4,000 factually unreliable, mixed-reliability, and factually reliable English-language news websites. Running our system over an 18 month period, we track the spread of 146K news stories. Using network-based interference via the NETINF algorithm, we show that the paths of news narratives and the stances of websites toward particular entities can be used to uncover slanted propaganda networks (e.g., anti-vaccine and anti-Ukraine) and to identify the most influential websites in spreading these attitudes in the broader news ecosystem. We hope that increased visibility into our distributed news ecosystem can help with the reporting and fact-checking of propaganda and disinformation.

==> dead.tex <==
\begin{table}
\centering
\scriptsize
\fontsize{6.5pt}{5pt}
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabularx}{1.0\columnwidth}{srrs}
\toprule
 {Keywords} & Articles &  Websites & Most Profilic Domains\\ \midrule
fed, inflation, hike, economist, rate  &32,273& 418 &theepochtimes.com (3,703), shornewsnetwork.com (3,507), dailymail.co.uk (2,774)  \\ \midrule
 desantis, ron, florida, governor, trump &22,968& 395 & dailymail.co.uk (1,701), washingtonexaminer (1,236), theepochtimes.com  (1,048) \\ \midrule

migrant, paso, border, patrol, crossing & 20,790 & 365 & dailymail.co.uk (2,655), nypost.com (1,872), breitbart.com (1,470) \\ \midrule
 
maralago, classified, fbi, raid, document & 20,742&374 & dailymail.co.uk (2,247), theepochtimes.com (1,534), nypost.com (1,470)  \\ \midrule
 iran, tehran, jcpoa, vienna, sanction & 19,540 & 314 & presstv.ir (2,665), tehrantimes.com(2,375), thenationalnews.com (1,160) \\ 

\bottomrule
\end{tabularx}
\caption{\label{tab:narratives} Top 5 narratives from unreliable news websites---by number of articles---in our dataset.} %\todo{how was this selection made? Sounds vague.
\end{table}


\section{JS-Divergence\label{sec:js-divergence}}
Formally JS-Divergence between two distributions P and Q is calculated as follows:
\begin{align*}
    JS(P||Q)&=\frac{1}{2}KL(P||\frac{(P+Q)}{2})+\frac{1}{2}KL(Q||\frac{(P+Q)}{2}) \\
    KL(P||Q)&=\sum_{x}P(x)\log(\frac{P(x)}{Q(x)})
\end{align*}
While performing stance We utilize this metric to evaluate the differences in the distribution between how unreliable and authentic news websites address a given entity/topic.



 2 & gucci, peta, handbag, dakota, crocodile & \tiny{Dakota Johnson has been criticized by PETA over a new Gucci campaign in which she's toting handbags made of reptile skins.  } &\tiny{Gucci isn't hiding it either, as its website touts the fact the hides are the real deal. That doesn't sit right with the animal rights org -- and it let Dakota know all about it in an informative, yet somewhat scathing, letter to her team. In the correspondence, obtained by TMZ, PETA takes issue with Gucci's python and crocodile handbags -- ranging from $3,100 to $31k -- being so unabashedly flaunted by Dakota ... which they say is odd, since she's outspoken on a lot of social issues. They're right, her IG is full of advocacy posts for everything from BLM to women's rights and a lot more."} \\\midrule

 3 & rolling, stone, daniel, exwife, debunked& \tiny{Rolling Stone’s ``Teddy Daniels'' hit piece is a smear job on par with the RussiaGate Piss Dossier paid for by Hillary Clinton in an effort to derail Trumps campaign and administration"}  &  \tiny{The National File can confirm that The Rolling Stone hit piece on Teddy Daniels is a smear job on par with the RussiaGate Piss Dossier paid for by Hillary Clinton in an effort to derail Trumps campaign and administration. National File is publishing this categorical fact check refuting Rolling Stones original article after reviewing multiple source documents related to thinly sourced and ultimately dubious claims made by Rolling Stone. The poorly sourced and thoroughly debunked Rolling Stone hitpiece attempted to paint Daniels as an abusive spouse who repeatedly failed to pay child support. Those claims have now been thoroughly debunked by National File.} \\ \midrule


 4 & sovereign, seminar, straight, citizen, guru&  \tiny{The Anti-Defamation League has accused one of the leading figures of the sovereign citizen movement, which claims that its members can break free of the regular legal system and become free-roaming American State Nationals if they just buy the right forms from him.} & \tiny{The group landed on law enforcements radar again in 2015, after its members sent faux-legal documents to a judge, prompting an FBI raid on a meeting. Story continues Straight, meanwhile, has become one of the leading figures of the sovereign citizen movement, often pushing his theories at multiple seminars a month where tickets can cost more than \$150. At his well-attended events, Straight rambles for hours about his oddball legal ideas, drawing complex diagrams on a white board and claiming that the American Bar Association is responsible for most of the problems in the United States. Straight has risen to become a sovereign citizen guru, according to the Anti-Defamation League, insisting that his followers can break free of the regular legal system and become free-roaming American State Nationals if they just buy the right forms from him.'.}\\ \midrule

5 & mchugh, whyno, tired, nhl, hockey& \tiny{ Get another cup of coffee because you need to have the same energy you had seven hours ago when we came on the air because the viewers don’t expect you to look tired, says the host of NBC’s Hockey Night in America.} & \tiny{And it is now two in the morning. So get another cup of coffee because you need to have the same energy you had seven hours ago when we came on the air because the viewers dont expect you to look tired, McHugh said. I think Im looking forward to those moments. Because in the end, those are the ones you remember. AP Hockey Writer Stephen Whyno contributed to this story. }\\\midrule

6  & saul, odenkirk, pudding, hasty, shady& \tiny{TBob Odenkirk, perhaps best known as shady lawyer Saul Goodman on Breaking Bad and Better Call Saul, has been named 2023 Man of the Year by Harvard University’s Hasty Pudding Theatricals.} & \tiny{ To honor the supporting role that entertainment journalism can play in this beloved pastime, The Associated Press on Thursday unveiled its inaugural AP Top 25 Movies ranking. Award-winning actor and writer and bestselling author Bob Odenkirk, perhaps best known as shady lawyer Saul Goodman on Breaking Bad and Better Call Saul, has been named 2023 Man of the Year by Harvard University's Hasty Pudding Theatricals} \\ \midrule

7 & ocasio-cortez, manford, dromm, jeanne, lgbtq&\tiny{Rep. Alexandria Ocasio-Cortez, D-New York, has sparked outrage with her suggestion that a post office in her Queens district be renamed in honor of a woman who cofounded the first organization for parents of gay and lesbian children in 1973 and her husband.} & \tiny{" Dromm said. "How dare she put our community's heritage up for a popularity contest or a vote," added Allen Roskoff, a longtime LGBTQ activist and head of the Jim Owles Liberal Democratic Club. Both Dromm and Roskoff told the Daily News that, while they generally support OcasioCortez and like her policies, "this is typical of her not being connected to the community.  }  \\\midrule


 8 & tumour, sheeran, diagnosed, ed, unbiased& \tiny{Ed Sheeran's wife was diagnosed with a tumour during her pregnancy, the singer has revealed.} & \tiny{Ed Sheeran wrote seven songs in four hours after his wife Cherry Seaborn was diagnosed with a tumour.} \\ \midrule


9 &mace, olbermann, hillary, clinton, hammer & \tiny{ Rep. Nancy Mace, R-S.C., tweeted that Hillary Clinton used a hammer to destroy evidence of a private e-mail server and classified information on that server and was never indicted.} & \tiny{Are you ok? You seem to have been hallucinating a lot lately. Keith Olbermann (@KeithOlbermann) June 11, 2023 Did he really want to go there? Fine: Fact. A hammer was used to destroy govt devices, and Hillary Clintons server was wiped out with a program called BleachBit, all fact checked by CNN (link below). Maybe your weed is stale.}\\\midrule

 10 & badge, black-owned, seller, amazon, chomp & \tiny{A new report found that Amazon gave small business and Black-owned business badges to companies that were neither.} &  \tiny{Amazon says the small business badge is for US companies with fewer than 100 employees and bringing in less than \$50 million in revenue. However, according to the report, companies like Black Rifle Coffee Co. received the badge despite generating over \$300 million in revenue in 2022. Sellers like beef jerky company Chomps received the Black-owned business badge despite its founders, Pete Maldonado and Rashid Ali, not being Black.}\\ 




 \subsection{Identifying and Understanding the Stance of New Narratives in the Misinformation News Ecosystem}
Having seen that by determining the overall stance of individual websites to particular keywords, we now show that by calculating the ratio between the week-over-week percentage increase in particular narrative volume among unreliable news websites and authentic news websites, we can determine which new news narratives are being spread primarily in unreliable news ecosystems. Then by determining the stance of these news narratives toward their extracted keywords, we can further determine how that particular narrative is approaching a given narrative or topic. We note that this programmatic can help determine which narratives are receiving new or renewed focus on {unreliable} news websites and which are addressing entities of interest in a particularly damaging manner allowing for the identification and amelioration of misinformation~\cite{rajdev2015fake, wu2019misinformation, saeed2022trollmagnifier,hanley2023specious}. 

Some of the narratives that had the largest relative increase amongst the unreliable news websites compared to the authentic news websites in the last week of our study (June 25 to July 1, 2023) were:

\vspace{3pt}
\noindent
\textbf{Pfizer Using Placebo Vaccines, Unreliable/Authentic Ratio: 14.0, Keywords: Pfizer, Batch, Danish, Bnt162b2, Adverse} 
The first narrative that was predominately spread throughout the unreliable news ecosystem concerned Danish scientists ostensibly discovering that batches of Pfizer vaccines were actually placebos. 
 \vspace{1pt}
\begin{displayquote}
\small
\textit{\textit{The Danish scientists uncovered “compelling evidence” that a significant percentage of the batches distributed in the EU likely consisted of “placebos and non-placebos,” prompting the researchers to call for further investigation.}}
\end{displayquote}
\vspace{1pt}

\noindent
We identified 14~news articles promoting this narrative, and performing stance detection, all except one had an anti-Pfizer stance.  The top domains that spread this narrative were sgtreport.com, theautomaticearth.com, and theburningplatform.com with two articles each. 

\noindent
\textbf{Ukrainian President Zelensky a Puppet, Unreliable/Authentic Ratio: 9.0, Keywords: Ukraine, MacGregor, Douglas, Colonel, Zelensky }:
The second narrative that predominantly spread in the unreliable news ecosystem concerned an interview with the retired US colonel Douglas Macgregor that suggested that the war between Ukraine and Russia was unwinnable and that Ukrainian President Zelenskey was a puppet of Western powers. 

\vspace{1pt}
\begin{displayquote}
\small
\textit{\textit{``The war is really over for the Ukrainians. I don’t see anything heroic about the man. And I think the most heroic thing he can do right now is to come to terms with reality," retired Army Colonel Douglas MacGregor told Fox Business News. "I think Zelensky is a puppet, and he is putting huge numbers of his own population in unnecessary risk," he said.}}
\end{displayquote}
\vspace{1pt}

\noindent Altogether, we identified nine articles about this particular news story in our dataset, and performing stance detection we identified six that had a negative Ukrainian stance, two that had a neutral stance, and one that had a positive stance. The top domain that spread this news story was paulcraigroberts.com (3 articles.com).


\vspace{3pt}
\noindent
\textbf{Government Censorship, Unreliable/Authentic Ratio: 8.0  Keywords: Censorship, Misinformation, Discredit, Loudan, Eiisac } 
The third narrative that predominantly spread within the unreliable news ecosystem concerned reports of US government censorship of Loudan County, Virginia. 


 \vspace{1pt}
\begin{displayquote}
\small
\textit{\textit{ The House Judiciary Committee released a report Monday detailing how election officials around the country tried to censor social media in the run-up to the 2022 midterm elections. In August 2022, a Loudoun County, Virginia, government official reported a Tweet featuring an unedited video of a county official because it was posted as part of a larger campaign to discredit the word of that official, the report notes. }}
\end{displayquote}
\vspace{1pt}

\noindent
Altogether, we identified eight articles from eight different websites including zerohedge.com, thedailycaller.com, and thegatewaypundit.com about this particular news story in our dataset, and by performing stance detection we identified that all had an anti-censorship stance. 


\begin{table}

\centering

\fontsize{7.5pt}{8}
%\small
\selectfont

\setlength\tabcolsep{4pt}

\begin{tabular}{lll|lll}
\textbf{}&\textbf{} & \textbf{} & \textbf{Predom. Misinfo} & \textbf{}  \textbf{}  \\ 
\textbf{All Narratives}&\textbf{Hub.} & \textbf{Eign.}  &\textbf{Narratives} &  \textbf{Hub} & \textbf{Eign.}  \\ \toprule
yahoo.com& 0.149 & 0.111&thegatewaypundit.com&0.129 &0.125\\

dailymail.co.uk &  0.101 & 0.099 & dailymail.co.uk& 0.075&0.054\\

apnews.com& 0.097 &0.092 &theburningplatform.com& 0.061 &0.022\\

independent.co.uk& 0.052 &0.097 &naturalnews.com & 0.060&0.028\\

nypost.com & 0.049& 0.075& theepochtimes.com& 0.057& 0.097 \\

cnn.com& 0.038 &0.070 &beforeitsnews.com& 0.048 &0.049\\

theepochtimes.com& 0.028&0.074 &ussanews.com& 0.036& 0.029\\

sandiegouniontribune.com&0.026& 0.057 &abovetopsecret.com& 0.089& 0.010\\

khon2.com & 0.060&0.053 &yahoo.com&  0.081  &0.013\\

washingtonpost.com& 0.023& 0.068 &breitbart.com & 0.081  &0.022\\

\bottomrule

\end{tabular}

\caption{\label{tab:most-influential-websites} Websites with the largest influence in the underlying influence graph determined by \texttt{NETINF} with (1) all narratives considered and (2) only narratives predominated by unreliable news websites.}

\end{table}



\begin{table*}
\begin{minipage}{.32\textwidth}
\centering
%\scriptsize
\fontsize{5.0pt}{1pt}
\setlength{\tabcolsep}{1pt}
\selectfont
\begin{tabular}{ll}
\multicolumn{2}{c}{\textbf{Abortion}} \\
\toprule
Pro Domains & Against Domains  \\ \midrule
cosmopolitan.com (59.4\%)  &patriotnewsalerts.com (96.4\%) \\
dw.com (57.7\%) &christiantoday.com(96.2\%) \\
hollywoodreporter.com (56.1\%) & campaignlifecoalition.com (94.9\%)\\
\bottomrule
\end{tabular}
\end{minipage}
\begin{minipage}{.32\textwidth}
\centering
%\scriptsize
\fontsize{5.0pt}{1pt}
\setlength{\tabcolsep}{1pt}
\selectfont
\begin{tabular}{ll}
\multicolumn{2}{c}{\textbf{Joe Biden}} \\
\toprule
Pro Domains & Against Domains  \\ \midrule
americanindependent.com (83.3\%) &americanjournaldaily.com (97.2\%) \\
wapt.com (81.6\%)& mediarightnews.com (96.8\%) \\
4029tv.com (80.8\%) & nationalreview.com (82.6\%)\\
\bottomrule
\end{tabular}
\end{minipage}
\begin{minipage}{.32\textwidth}
\centering
%\scriptsize
\fontsize{5.0pt}{1pt}
\setlength{\tabcolsep}{1pt}
\selectfont
\begin{tabular}{ll}
\multicolumn{2}{c}{\textbf{Donald Trump}} \\
\toprule
Pro Domains & Against Domains  \\ \midrule
chroniclesmagazine.org (42.9\%) &truthorfiction.com (100.0\%) \\
castanet.net (35.4\%)&13newsnow.com (100.0\%) \\
dailytorch.com( 35.0\%) & democracyguardian.com (100.0\%)\\
\bottomrule
\end{tabular}
\end{minipage}

\begin{minipage}{.32\textwidth}
\centering
%\scriptsize
\fontsize{5.0pt}{1pt}
\setlength{\tabcolsep}{1pt}
\selectfont
\begin{tabular}{ll}
\multicolumn{2}{c}{\textbf{Ukraine}} \\
\toprule
Pro Domains & Against Domains  \\ \midrule
jta.org (96.2\%) &theintercept.com (57.7\%) \\
emerging-europe.com (90.6\%)& conservativewoman.co.uk (55.9\%) \\
people.com (89.4\%) & thebulletin.org (54.1\%)\\
\bottomrule
\end{tabular}
\end{minipage}
\begin{minipage}{.32\textwidth}
\centering
%\scriptsize
\fontsize{5.0pt}{1pt}
\setlength{\tabcolsep}{1pt}
\selectfont
\begin{tabular}{ll}
\multicolumn{2}{c}{\textbf{Russia}} \\
\toprule
Pro Domains & Against Domains  \\ \midrule
popularresistance.org (27.5\%) &swissinfo.ch (100.0\%) \\
britannica.com (25.0\%)& towleroad.com (100.0\%) \\
thedispatch.com (24.1\%) & taskandpurpose.com (98.1\%)\\
\bottomrule
\end{tabular}
\end{minipage}
\begin{minipage}{.32\textwidth}
\centering
%\scriptsize
\fontsize{5.0pt}{1pt}
\setlength{\tabcolsep}{1pt}
\selectfont
\begin{tabular}{ll}
\multicolumn{2}{c}{\textbf{Vaccine}} \\
\toprule
Pro Domains & Against Domains  \\ \midrule
precisionvaccinations.com (99.2\%) &leicestermercury.co.uk (75.6\%) \\
financialexpress.com (98.7\%)& conservativewoman.co.uk (42.4\%) \\
aap.org (98.0\%) & amgreatness.com (41.7\%)\\
\bottomrule
\end{tabular}
\end{minipage}
\caption{\label{tab:authtenic-stance-websites} The set authentic news websites with the highest percentage of  \textit{Pro} and \textit{Against} articles about various entities/topics.}
\end{table*}

\begin{table*}
\begin{minipage}{.32\textwidth}
\centering
%\scriptsize
\fontsize{5.0pt}{1pt}
\setlength{\tabcolsep}{1pt}
\selectfont
\begin{tabular}{ll}
\multicolumn{2}{c}{\textbf{Abortion}} \\
\toprule
Pro Domains & Against Domains  \\ \midrule
newsbreak.com (35.8\%)  &evil.news (100.0\%) \\
hindustantimes.com (29.4\%) &gript.ie (100.0\%) \\
democraticunderground.com (26.0\%) & pop.org (98.1\%)\\
\bottomrule
\end{tabular}
\end{minipage}
\begin{minipage}{.32\textwidth}
\centering
%\scriptsize
\fontsize{5.0pt}{1pt}
\setlength{\tabcolsep}{1pt}
\selectfont
\begin{tabular}{ll}
\multicolumn{2}{c}{\textbf{Joe Biden}} \\
\toprule
Pro Domains & Against Domains  \\ \midrule
bipartisanreport.com (70.1\%) &stillnessinthestorm.com (100.0\%) \\
palmerreport.com (65.7\%)&thepatriotjournal.com (95.5\%) \\
occupydemocrats.com (65.7\%) & nationalinsiders.com (95.3\%)\\
\bottomrule
\end{tabular}
\end{minipage}
\begin{minipage}{.32\textwidth}
\centering
%\scriptsize
\fontsize{5.0pt}{1pt}
\setlength{\tabcolsep}{1pt}
\selectfont
\begin{tabular}{ll}
\multicolumn{2}{c}{\textbf{Donald Trump}} \\
\toprule
Pro Domains & Against Domains  \\ \midrule
roguereview.net (67.7\%) &newscorpse.com (95.6\%) \\
rsbnetwork.com (63.4\%)&whowhatwhy.org (93.9\%) \\
rubyraymedia.com (60.0\%) & politicususa.com (92.9\%)\\
\bottomrule
\end{tabular}
\end{minipage}

\begin{minipage}{.32\textwidth}
\centering
%\scriptsize
\fontsize{5.0pt}{1pt}
\setlength{\tabcolsep}{1pt}
\selectfont
\begin{tabular}{ll}
\multicolumn{2}{c}{\textbf{Ukraine}} \\
\toprule
Pro Domains & Against Domains  \\ \midrule
overpassesforamerica.com (73.3\%) &treason.news (89.2\%) \\
gbnews.uk (71.0\%)&expose-news.com (82.8\%) \\
thelondoneconomic.com (70.6\%) & newstarget.com(79.6\%)\\
\bottomrule
\end{tabular}
\end{minipage}
\begin{minipage}{.32\textwidth}
\centering
%\scriptsize
\fontsize{5.0pt}{1pt}
\setlength{\tabcolsep}{1pt}
\selectfont
\begin{tabular}{ll}
\multicolumn{2}{c}{\textbf{Russia}} \\
\toprule
Pro Domains & Against Domains  \\ \midrule
bigleaguepolitics.com(48.1\%) &politizoom.com (100.0\%) \\
whatreallyhappened.com (46.9\%)& wikispooks.com (97.8\%) \\
tass.com (46.7\%) & qresear.ch (96.9\%)\\
\bottomrule
\end{tabular}
\end{minipage}
\begin{minipage}{.32\textwidth}
\centering
%\scriptsize
\fontsize{5.0pt}{1pt}
\setlength{\tabcolsep}{1pt}
\selectfont
\begin{tabular}{ll}
\multicolumn{2}{c}{\textbf{Vaccine}} \\
\toprule
Pro Domains & Against Domains  \\ \midrule
news18.com (95.9\%) &dcdirtylaundry.com (69.2\%) \\
hindustantimes.com (93.6\%)& rubyraymedia.com (63.2\% \\
firstpost.com (88.0\%) &coronanews123.wordpress.com (62.9\%)\\
\bottomrule
\end{tabular}
\end{minipage}
\caption{\label{tab:misinformation-stance-websites} The set unreliable news websites with the highest percentage of  \textit{Pro} and \textit{Against} articles about various entities/topics.}
\end{table*}




\begin{table*}
\centering
\scriptsize
\fontsize{6.5pt}{5pt}
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabularx}{1.0\columnwidth}{srrs}
\toprule
 {Keywords} & Articles &  Websites & Most Profilic Domains\\ \midrule
desantis, ron, florida, gov, governor  &62,911&1,330 &yahoo.com (5,454),floridapolitics.com (3,098), thehill.com (1,900)  \\ \midrule
quarter, net, revenue, expense, loss &57,453& 824 & benzinga.com(19,266), yahoo.com (3,356), marketwatch.com  (3,106) \\ \midrule

half, halftime, minute, goal, possession &52,362 & 809 & yahoo.com (2,785), espn.com (2,527), rte.ie (2,124) \\ \midrule
 
symptom, fever, cough, throat, sore &42,581&1,241 & yahoo.com (1,685), webmd.com (1,023), news-medical.net (869)  \\ \midrule
roe, wade, abortion, dobbs, supreme& 38,358 & 1,317 & news-yahoo.com (2,118), thehill.com (798), cnn.com (615) \\ 

\bottomrule
\end{tabularx}
\caption{\label{tab:narratives} Top 5 narratives from our different types of news---by the number of articles---in our dataset.} %\todo{how was this selection made? Sounds vague.
\end{table*} %% Mainstream


\begin{table*}
\centering
\scriptsize
\fontsize{6.5pt}{5pt}
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabularx}{1.0\columnwidth}{srrs}
\toprule
 {Keywords} & Articles &  Websites & Most Profilic Domains\\ \midrule
desantis, ron, florida, gov, governor  &14,071&329 &dailymail.co.uk (2,831), ussanews.com (902), occupydemocrats.com (496)  \\ \midrule
dictatorship, democracy, censorship, propaganda, authoritarian
 &9,097& 359 & abovetopsecret.com (2,549), noqreport.com (384), theburningplatform.com (293)  \\ \midrule
respect, dignity, equal, equality, freedom
 &8,008 & 334 &dailymail.co.uk (3,090), abovetopsecret.com (2,183), lifesitenews.com (160)\\ \midrule
classified, document, maralago, archive, wilmington
 & 7,719&250 & dailymail.co.uk (1,393), thegatewaypundit.com (658), survivethenews.com (253)  \\ \midrule
constitution, oath, amendment, constitutional, defend
 & 7,664 & 354 &abovetopsecret.com (2,044), dailymail.co.uk (452), theqtree.com (307) \\  
\bottomrule
\end{tabularx}
\caption{\label{tab:narratives} Top 5 narratives from our different types of news---by the number of articles---in our dataset.} % Misinformation
\end{table*}


\begin{table*}
\centering
\scriptsize
\fontsize{6.5pt}{5pt}
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabularx}{1.0\columnwidth}{srrs}
\toprule
 {Keywords} & Articles &  Websites & Most Profilic Domains\\ \midrule
desantis, ron, florida, gov, governor  &32,615&385 &tampafp.com (1,762), theepochtimes.com (1,441), nypost.com (1,220)  \\ \midrule
half, halftime, minute, goal, possession
 &20,751& 227 & the-sun.com (2,402), thesun.co.uk (2,354), independent.co.uk (1,968)  \\ \midrule
kourtney, kardashians, travis, khloe, barker
 &19,180 & 116 &the-sun.com (7,046), thesun.co.uk (4,951), metro.co.uk (1,028)\\ \midrule
ronaldo, cristiano, portugal, football, manchester
 & 17,699&125 & the-sun.com (3,307), thesun.co.uk (3,024), dailystar.co.uk (1,732)  \\ \midrule
kardashians, khloe, kim, kourtney, jenner
 & 16,555& 144 &the-sun.com (5,603),thesun.co.uk (3,781), metro.co.uk (987) \\  
\bottomrule
\end{tabularx}
\caption{\label{tab:narratives} Top 5 narratives from our different types of news---by the number of articles---in our dataset.} % Misinformation
\end{table*}


\begin{table}

\centering

\fontsize{6.5pt}{8}
%\small
\selectfont

\setlength\tabcolsep{4pt}

\begin{tabular}{lll|lll}
\textbf{}&\textbf{} & \textbf{} & \textbf{Predom. Misinfo} & \textbf{}  \textbf{}  \\ 
\textbf{All Narratives}&\textbf{Hub.} & \textbf{Eign.}  &\textbf{Narratives} &  \textbf{Hub} & \textbf{Eign.}  \\ \toprule
yahoo.com& 0.149 & 0.111&thegatewaypundit.com& 0.129 &0.109\\

apnews.com &  0.101 & 0.092 & dailymail.co.uk& 0.075&0.125\\

dailymail.co.uk& 0.097 &0.099 &theburningplatform.com& 0.060 &0.103\\

nypost.com& 0.052 &0.076&naturalnews.com& 0.060&0.116\\

independent.co.uk & 0.049& 0.097& theepochtimes.com & 0.057& 0.116 \\

sandiegouniontribune.com& 0.037 &0.057&beforeitsnews.com&0.048 &0.117\\

cnn.com &  0.037 & 0.070 & ussanews.com& 0.036&0.124\\

khon2.com& 0.035 &0.053 &abovetopsecret.com& 0.028 &0.087\\

washingtonpost.com& 0.024 &0.068 &yahoo.com & 0.027&0.092\\

theepochtimes.com &0.023& 0.074& breitbart.com& 0.021& 0.077 \\

\bottomrule

\end{tabular}

\caption{\label{tab:most-influential-websites} Websites with the largest influence in the underlying influence graph determined by \texttt{NETINF} with (1) all narratives considered and (2) only narratives predominated by unreliable news websites.}

\end{table}


\begin{table}
\centering
\scriptsize
\fontsize{6.pt}{5pt}
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabularx}{1.0\columnwidth}{lr|lr|lr}
\toprule
 {Reliable} & Propor. &  Mixed &Propor. & Unreliable &Propor.\\ \midrule
kearneyhub.com & 0.414  &blacklistednews.com &  0.484 & tapnewswire.com  & 0.825 \\
bostonreview.net & 0.408 & churchmilitant.com &  0.452 & dcdirtylaundry.com  & 0.805 \\
theindependent.com & 0.372 & patriotnewsalerts.com & 0.374 & dcdirtylaundry.com & 0.756\\
biography.com & 0.372  & health.com &  0.360 & truth11.com 
 & 0.723\\
kxlf.com & 0.344 & conservativepapers.com & 0.356 & expose-news.com & 0.711 \\

 
\bottomrule
\end{tabularx}
\caption{\label{tab:narratives} Websites that pick up the most narratives --- as a percentage of their copies --- from the unreliable news ecosystem.} % 
\end{table}




\begin{table}

\centering

\fontsize{6.5pt}{8}
%\small
\selectfont

\setlength\tabcolsep{4pt}

\begin{tabular}{lll|lll}
\textbf{}&\textbf{} & \textbf{} & \textbf{Predom. Misinfo} & \textbf{}  \textbf{}  \\ 
\textbf{All Narratives}&\textbf{Hub.} & \textbf{Eign.}  &\textbf{Narratives} &  \textbf{Hub} & \textbf{Eign.}  \\ \toprule
yahoo.com& 0.149 & 0.111&thegatewaypundit.com& 0.129 &0.109\\

apnews.com &  0.101 & 0.092 & dailymail.co.uk& 0.075&0.125\\

dailymail.co.uk& 0.097 &0.099 &theburningplatform.com& 0.060 &0.103\\

nypost.com& 0.052 &0.076&naturalnews.com& 0.060&0.116\\

independent.co.uk & 0.049& 0.097& theepochtimes.com & 0.057& 0.116 \\

sandiegouniontribune.com& 0.037 &0.057&beforeitsnews.com&0.048 &0.117\\

cnn.com &  0.037 & 0.070 & ussanews.com& 0.036&0.124\\

khon2.com& 0.035 &0.053 &abovetopsecret.com& 0.028 &0.087\\

washingtonpost.com& 0.024 &0.068 &yahoo.com & 0.027&0.092\\

theepochtimes.com &0.023& 0.074& breitbart.com& 0.021& 0.077 \\

\bottomrule

\end{tabular}

\caption{\label{tab:most-influential-websites} Websites with the largest influence in the underlying influence graph determined by \texttt{NETINF} with (1) all narratives considered and (2) only narratives predominated by unreliable news websites.}

\end{table}


\begin{table}

\centering

\fontsize{7.5pt}{8}
%\small
\selectfont

\setlength\tabcolsep{4pt}

\begin{tabular}{llll}
&\textbf{Feature} &  &\textbf{Authentic \% -} \\ 
\textbf{Stance-Topic}&\textbf{Importance} & \textbf{JS-Divergence} &\textbf{Unreliable \%} \\ \toprule

Pro\_Joe\_Biden &  0.0146 & 0.217 & 0.243\\
Pro\_Ukraine & 0.0142 & 0.146 &0.163\\
Pro\_mifepristone & 0.0132 & 0.243 & 0.297\\
Pro\_abortion & 0.0128& 0.172 &0.148\\
Against\_Donald\_Trump & 0.0127& 0.085 & 0.077\\
Neutral\_immigration & 0.0124 & 0.145 &0.123\\
Against\_vaccine &  0.0110 & 0.246 &-0.253\\
Pro\_vaccine & 0.0100 &  0.246 & 0.308\\
Pro\_roe\_v\_wade & 0.0099 &  0.100 & 0.081\\
Pro\_medicaid & 0.0081 & 0.172 & 0.170\\
\bottomrule

\end{tabular}

\caption{\label{tab:largest-diff-increase}The most informative topics that differentiate unreliable news websites from authentic news websites. }

\end{table}


\subsection{Stances to Popular Entities and Topics}
To ensure the efficacy of our approach, and to understand the attitudes of our set of websites to several popular topics, we plot the percentage of news articles that had a particular stance to several popular entities among our top topics including \textit{Donald Trump, Joe Biden, Abortion,  Russia, Ukraine, and Vaccines}. We plot additional topics including \textit{Immigration, Artificial Intelligence, Ron Desantis, Israel, and China} in Appendix~\ref{sec:additional-stances}. To make these stance percentages more robust over time, we predict the stance of all passages whose respective clusters include these topics within the top ten PMI keywords. 

Analyzing the stances on domain basis, using political polarization data for our set of websites from Robertson et~al~\cite{robertson2018auditing}, which grades the US-based partisanship of websites between -1 (liberal/Democratic-leaning) and +1 (conservative/Republican-leaning), we find that there is a 0.588/-0.518 correlation between the percentage of website's articles that are \textit{Pro}/\textit{Against} the for Republican US President Donald Trump. Finding the individual narrative cluster with the highest percentage of pro-Trump articles, we find it to be a set of articles about Donald Trump's speech celebrating Abraham Lincoln with the  auto-generated summary:

%\begin{displayquote}
%\small
%\textit{If Democrats thought their indictments of Donald Trump were going to derail his campaign, they were sorely mistaken. For years, Democrats have waged a propaganda campaign to tarnish Trump's reputation with Americans. Despite this, Trump continues to win the hearts and minds of Americans across the country. Just recently, he attended a Lincoln Day Dinner at a crucial battleground state in the upcoming election. The former president is hot on the campaign trail. The crowd roared with approval at nearly everything he said.}
%\end{displayquote}

\noindent
Similarly, we find a -0.752/0.796 correlation between the percentage of a website's articles that are \textit{Pro}/\textit{Against} current Democratic US President Joe Biden. Finding the individual narrative cluster with the highest percentage of pro-Joe Biden articles, we find it to be a set of articles about Joe Biden's positive perception in Ireland with the summary:

% \begin{displayquote}
%\small
%\textit{The Irish response to Biden has been overwhelmingly positive for "Cousin Joe," as many have called him. In Dundalk and Ballina, Knock and Dublin, thousands of people waited nearly eight hours to see him. As he made his way through streets filled with admirers, some strained to get even a touch from him. Biden visited five countries on a single trip to the continent in 2008, touting his accomplishments at a time of domestic backlash.}
%\end{displayquote}
%\noindent











Furthermore, as seen in Figures~\ref{fig:percentage-stance-authentic}
and~\ref{fig:percentage-stance-unreliable}, throughout our period of study we observe relatively stable stances towards each of our chosen entities from authentic and unreliable news websites. We find that the articles of unreliable news websites are more pro-Donald Trump (absolute 7.9\% more), anti-Joe Biden (29.4\% more), anti-abortion (18.7\% more), pro-Russia (5.8\% more), anti-Ukraine (18.6\%), and anti-vaccine (25.4\%). Finally, examining the particular websites with the highest percentage of \textit{Pro} and \textit{Against} articles for Joe Biden, Donald Trump, vaccines, Russia, Ukraine, and abortion, we find a relatively predictable set of sites (Tables~\ref{tab:authtenic-stance-websites} and~\ref{tab:misinformation-stance-websites}) For example, one of the most pro-Russia as seen in Table~\ref{tab:misinformation-stance-websites}, is tass.com, Russia's state-owned news agency~\cite{center2020pillars}.  We note, as seen in Figures~\ref{fig:percentage-stance-authentic} and~\ref{fig:percentage-stance-unreliable} that the amount of Pro-Ukraine (16.8\% absolute increase) and Anti-Russian articles (32.9\%) spiked following the Russian invasion of Ukraine in February 2022. We further find that one of the most anti-vaccine websites is the unreliable news website coronanews123.wordpress.com. Altogether this illustrates our approach's ability to extract the overall stance of websites to particular entities.

\subsection{Predicting Reliability of Websites Using Stance}
Having seen the divergent views toward several popular entities in our dataset from unreliable and authentic news websites, we now determine whether a website's attitude toward particular entities (\textit{e.g.}, vaccines), can be utilized to differentiate between authentic news and unreliable news websites. To do so, we gather the stances of each of our websites to the top 1,000 narratives within our dataset (\textit{i.e.}, the percentage of the website's articles that are \textit{Pro,} \textit{Against}, and \textit{Neutral} to extract topic-keyword of the narrative), we subsequently fit a random forest classifier to 80\% (3261~websites) of the websites' stance data (using 10\% of the websites as validation (408~websites), 10\% as test data). Based on the stances alone to these particular keywords, we achieved a 0.923 AUC in labeling the set of websites from our test dataset as unreliable vs. authentic. 

Our approach is highly interpretable, as we can determine which features are most important for distinguishing between unreliable and authentic websites (similarly if we wish to only find, for instance, anti-vaccine unreliable websites, our approach could focus only on that topic as well). We list the most important features that found to be distinctive between our set of unreliable and authentic news websites in Table~\ref{tab:largest-diff-increase}. In addition to displaying the feature importance outputted by our model, we further list the difference in raw percentage for articles that have the stance feature between our set of authentic news websites and unreliable news websites as well as the JS-Divergence between authentic news websites' stance distribution and unreliable news websites' stance distribution (a metric for determining the similarity of distributions, where a value of 0 means complete similarity and a value of 1 means complete divergence) for the feature. Some of the most distinctive features  (Table~\ref{tab:largest-diff-increase}) that distinguish between unreliable and authentic news websites include support for Joe Biden, support of abortion drugs like mifepristone,\footnote{\url{https://web.archive.org/web/20230104030044/https://www.fda.gov/drugs/postmarket-drug-safety-information-patients-and-providers/questions-and-answers-mifepristone-medical-termination-pregnancy-through-ten-weeks-gestation}} and being against vaccines. 


\begin{figure}
  \centering
  \includegraphics[width=1\columnwidth]{figures/contrastive_precision_recall_training2.pdf}
\caption{Evaluation of our model's precision, recall, and $F_1$ scores on the English portion of the English portion of SemEval22 test dataset~\cite{goel2022semeval} (using 3.0 as the cut-off for the two articles being about the same event~\cite{hanley2022partial}).
}
\label{fig:semeval-study}
\end{figure}



\begin{table}[ht]
\centering
\small
\begin{tabularx}{1\columnwidth}{lr}
\toprule
\textbf{Reliable} & \textbf{Propor.} \\
\midrule
yahoo.com          & 0.010 \\
apnews.com         & 0.008 \\
abcnews.go.com     & 0.007 \\
\midrule
\textbf{Mixed Reliability} & \textbf{Propor.} \\
\midrule
yahoo.com          & 0.015 \\
cnn.com            & 0.008 \\
abcnews.go.com     & 0.008 \\
\midrule
\textbf{Unreliable} & \textbf{Propor.} \\
\midrule
yahoo.com          & 0.014 \\
cnn.com            & 0.006 \\
apnews.com         & 0.006 \\
\bottomrule
\end{tabularx}
\caption{\label{tab:reliable-common-copy} For each news ecosystem, the reliable news websites that are the most often copied/influential.}
\end{table}


 \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/articles_negative_to_ukraine-20240902.pdf}
        \caption{Dist. of Against Ukraine Articles}
        \label{fig:d4-dimensions}
    \end{subfigure}

        \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/articles_negative_to_vaccines-20240902 (3).pdf}
        \caption{Dist. of Against Vaccines Articles}
        \label{fig:d4-dimensions}
    \end{subfigure}

\begin{minipage}{.45\textwidth}
\centering
%\scriptsize
\small
\setlength{\tabcolsep}{1pt}
\selectfont
\begin{tabular}{lll}
\multicolumn{3}{c}{\textbf{Pro Artificial Intelligence}} \\
\toprule
Reliable & Mixed & Unreliable \\ \midrule
prnewswire.com (95.5\%) & gulfnews.com (73.7\%)  & abovetopsecret.com (56.0\%)  \\ 
goodmenproject.com (84.2\%) & techstartups.com (57.9\%)  & technocracy.news (46.2\%)  \\ 
singularityhub.com (76.2\%) & thesun.co.uk (53.3\%)  & dailymail.co.uk (41.5\%)  \\ \bottomrule
\multicolumn{3}{c}{\textbf{Against Artificial Intelligence}} \\
\toprule
Reliable & Mixed & Unreliable \\ \midrule
rollingstone.com (52.9\%) & headtopics.com (28.4\%)  & activistpost.com (35.7\%)  \\ 
theweek.com (50.0\%) & dailystar.co.uk (28.0\%)  & naturalnews.com (30.0\%)  \\ 
slate.com (46.7\%) & uproxx.com (23.8\%)  & freedomsphoenix.com (27.3\%)  \\ 
\bottomrule
\end{tabular}
\end{minipage}

\begin{minipage}{.5\textwidth}
\centering
%\scriptsize
\small
\begin{tabular}{lll}
\multicolumn{3}{c}{\textbf{ Pro Kamala Harris}} \\
\toprule
Reliable & Mixed & Unreliable \\ \midrule
amsterdamnews.com (66.7\%) & jns.org (60.0\%)  & thinkamericana.com (72.1\%)  \\ 
liveuamap.com (66.7\%) & policetribune.com (57.1\%)  & dailypoliticalnewswire.com (69.3\%)  \\ 
biography.com (63.6\%) & thetrumpet.com (57.1\%)  & theunionjournal.com (43.5\%)  \\ 
\multicolumn{3}{c}{\textbf{Against Kamala Harris}} \\
\toprule
Reliable & Mixed & Unreliable \\ \midrule
mtstandard.com (78.9\%) & arizonadailyindependent.com (85.7\%)  & greatamericandaily.com (64.3\%)  \\ 
nola.com (70.0\%) & punchingbagpost.com (84.6\%)  & nextnewsnetwork.com (64.3\%)  \\ 
capoliticalreview.com (65.2\%) & renewedright.com (84.2\%)  & neonnettle.com (61.5\%)  \\ 
\bottomrule
\end{tabular}
\end{minipage}

\begin{minipage}{.5\textwidth}
\centering
\small
\begin{tabular}{lll}
\multicolumn{3}{c}{\textbf{ Pro Donald Trump}} \\
\toprule
Reliable & Mixed & Unreliable \\ \midrule
chicagoreader.com (41.2\%) & capitalresearch.org (33.3\%)  & focusonthefamily.com (34.5\%)  \\ 
thebaffler.com (33.3\%) & mondoweiss.net (30.0\%)  & stonecoldtruth.com (34.4\%)  \\ 
sandiegoreader.com (31.4\%) & arizonadailyindependent.com (29.2\%)  & nationalrighttolifenews.org (33.3\%)  \\ 
\bottomrule

\multicolumn{3}{c}{\textbf{Against Donald Trump}} \\
\toprule
Reliable & Mixed & Unreliable \\ \midrule
nationalobserver.com (78.6\%) & themilitant.com (72.7\%)  & brandnewtube.com (91.7\%)  \\ 
accountable.us (70.0\%) & trendingviews.co (64.3\%)  & kunstler.com (84.6\%)  \\ 
independent.org (66.7\%) & newshounds.us (60.0\%)  & theamericanreport.org (72.7\%)  \\
\bottomrule
\end{tabular}
\end{minipage}
    
\begin{minipage}{.5\textwidth}
\centering
\small
\begin{tabular}{lll}
\multicolumn{3}{c}{\textbf{ Pro America}} \\
\toprule
Reliable & Mixed & Unreliable \\ \midrule
messengernews.net (100.0\%) & bluegrasstimes.com (100.0\%)  & adflegal.org (100.0\%)  \\ 
nationalgeographic.com (100.0\%) & tribunnews.com (100.0\%)  & worldcouncilforhealth.org (100.0\%)  \\ 
fee.org (100.0\%) & yaf.org (100.0\%)  & nvic.org (100.0\%)  \\    \\ 
\bottomrule
\multicolumn{3}{c}{\textbf{ Against America}} \\
\toprule
Reliable & Mixed & Unreliable \\ \midrule
thepeoplescube.com (100.0\%) & thepatriotjournal.com (76.9\%)  & infostormer.com (80.0\%)  \\ 
cjr.org (50.0\%) & greanvillepost.com (68.9\%)  & paulcraigroberts.org (71.4\%)  \\ 
techdirt.com (46.2\%) & newscorpse.com (58.8\%)  & gellerreport.com (64.9\%)  \\ 
\bottomrule
\end{tabular}
\end{minipage}

 \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/articles_psitive_to_ai-20240902.pdf}
        \caption{Dist. of Pro AI}
        \label{fig:d4-dimensions}
    \end{subfigure}


        \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/articles_positive_to_harris-20240902.pdf}
        \caption{Dist. of Pro Kamala Harris}
        \label{fig:d4-dimensions}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/articles_positive_to_trump-20240902.pdf}
        \caption{Dist. of Pro Donald Trump}
        \label{fig:d4-dimensions}
    \end{subfigure}

       \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/articles_negative_to_harris-20240902.pdf}
        \caption{Dist. of Against Kamala Harris}
        \label{fig:d4-dimensions}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/articles_negative_to_trump-20240902.pdf}
        \caption{Dist. of Against Donald Trump}
        \label{fig:d4-dimensions}
    \end{subfigure}

     \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/articles_negative_to_ai-20240902.pdf}
        \caption{Dist. of Against AI}
        \label{fig:d4-dimensions}
    \end{subfigure}


    % On average, each embedding had an average similarity of 0.642 to its cluster center a each story cluster had an average cosine similarity of 0.021 with other identified story clusters


    
%Recent work within the security community has attempted to solve this issue by likening misinformation to spam, phishing, or government censorship. As such the community has attempted to reduce the spread of misinformation through tracking~\cite{hanley2023specious}, security warnings~\cite{kaiser2021adapting}, and account and website classification~\cite{hounsel2020identifying,paudel2023lambretta,saeed2022trollmagnifier}. However, many of these approaches, either fail to scale to the quick and viral pace of misinformation, rely on deep-learning techniques that are often not human-interpretable and that fail to generalize well to stories outside of their training domains, or do not take into account the full news ecosystem that supports misinformation~\cite{hanley2023specious,starbird2018ecosystem, wu2019misinformation,zannettou2019disinformation}. Furthermore, due to recent restrictions on the study of social media platforms, many past approaches are no longer possible~\cite{Cursino2023,Reddit2023}. Similarly, qualitative approaches, primarily conducted through human-intensive analysis~\cite{prochaska2023mobilizing,plasser2005hard}, which seek to identify larger trends further often remain limited in scope.


==> twitter-emily.tex <==
\section{Fact-Checking: Efficacy of Community Driven Efforts vs. News Organizations} As previously seen, using our system, we can identify potentially new unreliable news narratives. Once identified, traditionally two approaches to address the spread of these narratives have been relying on news organizations~\cite{factcheck-wapo} for fact-checking and community-driven fact-checking~\cite{wojcik2022birdwatch}. In this section,  we (1) exhibit how our system can be utilized for systematically identifying previously fact-checked information on unreliable news websites and  (2) further compare the efficacy of news organization and community-driven fact-checking. Specifically, after determining how long particular narratives spread in amongst our set of unreliable news websites before being fact-checked, we determine the fact-checking efficacy of news organizations Politifact~\cite{politifactFactCheck2022} and Reuters~\cite{reutersFactCheck2022} and compare them against the fact-checking ability of the community-driven fact-checking on Twitter Community Notes~\cite{wojcik2022birdwatch}.

 We augment our system to perform fact-checking  (\textit{i.e.}, determine whether a fact-check article \emph{refutes} a given narrative) by training a Natural Language Inference (NLI)-based system~\cite{zlatkova2019fact,nyhan2010corrections,rashkin2017truth} to ascertain when a claim from an article is refuted by a Twitter Community note or by the fact-checking reporting of Politifact or Reuters. To do so we fine-tune a DeBERTa-v3-based~\cite{he2022debertav3} classifier on the FEVER~\cite{thorne2018fever} and VitaminC fact-checking datasets~\cite{schuster-etal-2021-get}. This classifier takes a query/claim (\textit{i.e.}, an article) and a document (\textit{i.e.}, a fact-check) and labels the document as either \textit{supporting} the claim, \textit{refuting} the claim, or \textit{not having enough information} to say anything about the claim.  Using 10\% of the FEVER and VitaminC datasets as a held-out test set, our DeBERTa-based model achieves an overall 90.0\% $F_1$-score on this test set (96.9\% precision in labeling supporting statements and 90.8\% precision in labeling refutations). 


For Politifact and Reuters, we gathered the set of fact-checking articles that each published between January 1, 2022, and July 1, 2023. We then subset these articles to the set of Politifact articles that labeled claims as ``Mostly False'', ``False'', and ``Pants on Fire'' and the set of articles where Reuters labeled a claim as ``False''.  Altogether we gathered a set of 2,459 articles from Politifact and 1,052 articles from Reuters that fit this criterion. In addition, between  January 1, 2022, and June 30, 2023, we collected the set of Twitter Community Notes that were published daily on Twitter\footnote{\url{https://twitter.com/i/communitynotes/download-data}} as well as the corresponding fact-checked Tweets (on June 30, Twitter began restricting access to viewing tweets~\cite{Cursino2023}). We subset these community notes to those that were labeled as ``misinformed or potentially misleading’’ and were not fact-checking a visual media (image or video)  Altogether, we collected  46,083 community notes and their corresponding tweets.  We note that for all tweets and articles, we performed the preprocessing outlined in Section~\ref{sec:preprocess} and removed hashtags from our set of tweets. 

For each fact-checking article, we divide the article into its constituent passages, identifying the passage that refuted the claim being fact-checked (typically the last passage/paragraph in the article for both Politifact and Reuters fact-checking articles) and embed that passage using our \texttt{e5-base-v2} model. Similarly, for each Twitter community note, we identify the community-noted tweets and similarly embed them. For each article and tweet, we then map each fact-check passage to the narrative with the highest cosine similarity to the given passage/tweet. After mapping these fact-checking passages/tweets to our set of articles narrative, for each passage, we utilize our DeBERTa-v3-classifier to identify the set of article passages that were from our set of unreliable news websites that were \emph{refuted} by the fact-checking article. Conversely, we identify the set of news article passages from our set of unreliable news websites that agreed with or were \emph{supported} by the community-noted ``misinformed or potentially misleading’’ tweet (and thus fact-checked by the Twitter Community Note). Taking a subset of 292 different fact-checks, we find that our system maintained its performance under this system, finding that it had 88\% precision in correctly labeling refuting, and supporting statements.

Upon identifying fact-checked narratives, we find that on average, in the first week that they appeared on their corresponding unreliable news websites, the ratio of unreliable news articles to authentic news articles was 1.96 for PolitiFact, 2.05 for Reuters, and 2.29 for Twitter Community Notes. This indicates that a ratio of 2 may be a good ratio for identifying unreliable narratives using our system. Across all three fact-checkers, only 12.0\% of the narratives with a ratio greater than 2 were fact-checked.



\begin{table}
\centering
\setlength\tabcolsep{5pt}
\scriptsize
\begin{tabular}{lllll}
\toprule
  &Avg.    &Avg.  &  Avg. \%   \\ 
  &Art. Prior   & {Days to }  &{of Narrative  }     \\ 
 &Fact-Check   & {Fact-Check} &{Already Spread } \\ \midrule
Politifact  &36.8 &64.1&  30.6\% \\
Reuters  &35.8& 49.8 & 45.3\%\\
Community Notes &  60.7 &92.8 & 47.3\%\\
\bottomrule
\end{tabular}
\caption{\label{tab:fact-check} The estimated efficacy of fact-checking websites for different fact-checking organizations. } 
\end{table}



\begin{figure}
  \centering
  \includegraphics[width=0.9\columnwidth]{figures/factcheck3_to_misinformation.pdf}
\caption{ The percentage of narrative spread on misinformation websites before being fact-checked by Politifact, Reuters, and  Twitter Community Notes. }

\label{fig:rate-of-narrative-srpead-factcheck}
\end{figure}



As seen in Table~\ref{tab:fact-check}, while on average many narratives can spread throughout the news article ecosystem on the order of months, many narratives are immediately fact-checked by Politifact, Reuters, and Twitter Community Notes. Indeed as seen in Figure~\ref{tab:fact-check}, at the high end, nearly 51.8\% of the narrative fact-checked by Politifact in our dataset were fact-checked the day that a corresponding article spreading the false claim was seen in our dataset. However, while many fact-checkers \emph{are} effective at fact-checking narratives before they spread throughout the news ecosystem, on average, other narratives can spread for months before being fact-checked. 

Comparing Politifact, Reuters, and Twitter Community Notes, we find that while Twitter Community fact-checked the most claims with over 46K different tweets (compared to 2.6K from Poltiifcat and 1K from Reuters fact-checks), on average, the Twitter Community Notes were the least effective at fact-checking false claims as they appeared within the ecosystem. As shown in Table~\ref{tab:fact-check}, seen in Figure~\ref{fig:rate-of-narrative-srpead-factcheck}, and confirmed by performing a Mann-Whitney U-test, Twitter Community notes fact-checks at a slower rate than Politifact (statistically insignificant difference between Reuters and Twitter Community Notes according to the Mann-Whitney U-test).
